InstructRAG: Leveraging Retrieval-Augmented Generation on Instruction Graphs for LLM-Based Task Planning

Recent advancements in large language models (LLMs) have enabled their use as agents for planning complex tasks. Existing methods typically rely on a thought-action-observation (TAO) process to enhance LLM performance, but these approaches are often constrained by the LLMs' limited knowledge of complex tasks. Retrieval-augmented generation (RAG) offers new opportunities by leveraging external databases to ground generation in retrieved information. In this paper, we identify two key challenges (enlargability and transferability) in applying RAG to task planning. We propose InstructRAG, a novel solution within a multi-agent meta-reinforcement learning framework, to address these challenges. InstructRAG includes a graph to organize past instruction paths (sequences of correct actions), an RL-Agent with Reinforcement Learning to expand graph coverage for enlargability, and an ML-Agent with Meta-Learning to improve task generalization for transferability. The two agents are trained end-to-end to optimize overall planning performance. Our experiments on four widely used task planning datasets demonstrate that InstructRAG significantly enhances performance and adapts efficiently to new tasks, achieving up to a 19.2% improvement over the best existing approach.

==> rebuttal.tex <==
== Response to Reviewer 2x2g ==

Thank you for the constructive suggestions. We appreciate your recognition that our work achieves notable performance improvements.

**(1) What is the scope of the existing instructions (nodes) in the instruction graph? If entirely new tasks or instructions emerge, can InstructRAG still maintain its claimed enlargability to adapt effectively?**

The instruction graph encompasses the instructions within the scopes of the support sets, as summarized in Table 1. We conduct an experiment using the ScienceWorld dataset, where the trained InstructRAG model (originally trained on HotpotQA) is applied directly to ScienceWorld tasks. These tasks are entirely new to the InstructRAG. The results are reported below. Following [19], we evaluate effectiveness using a dense reward function ranging from 0 to 1, with higher values indicating better performance. We observe that InstructRAG consistently outperforms the best baseline method, RAP, achieving improvements of approximately 6%-10%.

| Backbone     | Method | ScienceWorld |
|------------------|--------------------|----------------|
| GLM-4 | RAP              |     24.37      |
|  | InstructRAG      |     26.85      |
|GPT-4o mini  | RAP  |       23.49    |  
|  | InstructRAG      |    25.10       |
| DeepSeek-V2 | RAP              |   32.15        |
|  | InstructRAG      |       33.96    |


**(2) Does the system remain robust in the presence of noisy data? For example, could erroneous historical paths in the instruction graph compromise the system's reliability or degrade task performance?**

We incorporate erroneous historical paths into the Instruction Graph based on the provided comments, with the number of paths controlled by a noise rate ranging from 10% to 50%. For comparison, we use RAP, the best baseline method as a reference, which also includes noisy paths in its database. The F1 score results, based on DeepSeek-V2 for HotPotQA, are reported below. Notably, even with a noise rate of 50%, performance remains relatively stable, with only a 11.1% decrease. This robustness stems from the diverse instruction combinations that help select appropriate paths and mitigate noise effectively.

| Noise rate| 0% | 10% | 20% | 30% | 40% | 50% |
|-----------|-----------|-----------|-----------|-----------|-----------|-----------|
|RAP| 29.82 | 28.74 | 27.42 | 26.01 | 24.10 | 21.72 |
InstructRAG| 37.17 | 36.64  |  36.17 | 35.45 | 34.29 | 33.04|

**(3) The experimental metrics are overly narrow, focusing on limited aspects of task performance, and the baselines compared are insufficient to fully establish InstructRAG's superiority; more diverse and comprehensive comparisons are necessary to robustly validate the effectiveness of InstructRAG.**

To ensure more diverse and comprehensive comparisons, we explore i) a new language backbone (Mistral 7B), ii) introduce additional evaluation metrics (accuracy on HotpotQA and success rate on Webshop) following [12, 22], and iii) a typical baseline method, CoT-SC, and we note that many other baseline methods have been surpassed by the selected baselines reported in this paper. Below, we present our results alongside the best baseline method, RAP, for comparison. We note that InstructRAG demonstrates robust effectiveness across various backbone LLMs and evaluation metrics.

| Backbone     | Method | HotpotQA (Acc) | Webshop (Success Rate) |
|------------------|--------------------|----------------|----------------|
| Mistral 7B | CoT-SC           |      21.50     |    30.00     |
|            | RAP         |     22.87      |    40.83     |
|            | InstructRAG         |    27.99       |     43.33    |

== Response to Reviewer JUsN ==

Weaknesses:
**(1) What is "Few-shot time"? This concept is not explained in the paper. Additionally, the statement, "a task requires 27.1 minutes for adaptation," is unclear. Where can this be observed in the results?**

"Few-shot time" refers to the time of the few-shot learning stage in meta-learning, as summarized in Table 1. During this stage, we update the parameters of the two trained agents for each unseen task using a few-shot examples. The time cost is reported based on the number of unseen tasks or the number of samples per task, as shown in Figure 2. Furthermore, we report the average few-shot time per task, which is 27.1 minutes. This value is derived from the data in Figure 2.

**(2) It is challenging to compare the proposed model with baselines. For example, the authors report F1 scores of 27–33% for HotPotQA using various backbone LLMs, whereas GenGround reports 52.26% in the original paper using Mistral 7B. While it is understandable that identical LLMs might not always be available, the performance gap warrants further discussion.**

We clarify that the performance gap arises from three factors: (i) the 52.26% reported in the original paper is based on GPT-3.5-turbo-instruct, which is more powerful than the three LLMs examined in this study; (ii) our experiments evaluate transferability, where the model is trained on seen tasks and tested on unseen tasks, making the results naturally more challenging than those in the original paper; and (iii) the original models are not open-source (despite our efforts to contact the authors), so we reimplemented them to the best of our ability, ensuring a fair comparison, such as using the same retriever (LlamaIndex) as in our setup.

**(3) There is no significance testing provided for the results. Are the improvements reported in Table 2 (compared to baselines) and Table 4 (ablation study) statistically significant?**

Yes, Tables 2 and 4 are statistically significant, as confirmed by a t-test with p < 0.05. This is noted in Footnote 2 on page 7.


**(4) The results section requires considerable expansion. Crucial tables, such as key results, are placed in the appendix, which is not acceptable; the paper must be self-contained in its main body.**

Thank you for the suggestion. In the final version, we will include key tables (e.g., Table 5 and Table 6) in the main body.


== Response to Reviewer rTAg ==

**(1) The experiments primarily focus on three conventional tasks. Has there been consideration of the generalization capabilities across a broader range of task types or datasets? Is the performance improvement consistent across all tasks, or is it more pronounced in specific types of tasks?**

We note that the three tasks examined in this paper have been widely adopted in existing agent planning studies [40, 19, 23, 12, 22, 41], encompassing a diverse range of applications, including Wikipedia QA, embodied tasks, and Web shopping. To further evaluate the generalization capabilities of InstructRAG, we apply the model trained on HotpotQA to tasks from the ScienceWorld dataset. These tasks assess agents' scientific reasoning abilities at an elementary school science curriculum level and are entirely novel to the trained model. The results are presented below. The performance improvement remains consistent across tasks, achieving approximately 6%-10% higher results compared to RAP.

| Backbone     | Method | ScienceWorld |
|------------------|--------------------|----------------|
| GLM-4 | RAP              |     24.37      |
|  | InstructRAG      |     26.85      |
|GPT-4o mini  | RAP  |       23.49    |  
|  | InstructRAG      |    25.10       |
| DeepSeek-V2 | RAP              |   32.15        |
|  | InstructRAG      |       33.96    |


**(2) How does InstructRAG achieve rapid adaptation to new tasks? How efficient is its learning on new tasks?**

We explore meta-learning to train InstructRAG, aiming to develop adaptable parameters that can rapidly adjust to new tasks, aligning with the principles of meta-learning. To demonstrate the efficiency of task learning, we present the results in Figure 2, showing the time cost relative to the number of unseen tasks. On average, adapting to a new task takes 27.1 minutes.

**(3) The motivation presented is insufficient, lacking a comprehensive analysis of existing methods. The paper does not adequately explain why current approaches fail to meet these requirements or why InstructRAG is a necessary improvement rather than an optional one. Furthermore, the experimental section could benefit from a more in-depth analysis of why RAP produces incorrect answers, clearly differentiating the improvements and distinctions of InstructRAG compared to other methods.**

To the best of our knowledge, this paper is the first to study the two requirements of enlargability and transferability. Regarding enlargability, existing methods (e.g., RAP) retrieve past trajectories stored in an external database but do not address the combination of instructions within these trajectories. Intuitively, combining instructions can expand database coverage and create new paths not present in the pre-built database. The effectiveness of this property has been evaluated both quantitatively (Tables 2-3) and qualitatively (Tables 10-12). Regarding transferability, training agents to develop planning capabilities that adapt to new tasks remains beyond the scope of existing methods.

In the experimental section, we analyze the planning results of RAP, as shown in Table 10. InstructRAG demonstrates an advantage by combining two paths based on a common instruction, search[Piers Haggard]. This approach effectively links two key items—Anthony Minghella, representing the novel, and Piers Haggard, representing the film adaptation of "The Talented Mr. Ripley". These connections enable the LLM to generate a correct query formulation, allowing it to retrieve information about the film director within the generated thoughts (e.g., Thought 5). In contrast, RAP struggles to produce a correct query based on its retrieved experiences. Its generated thoughts fail to support effective query formulation, often resulting in a planning deadlock.

**(4) While the paper lists baseline models, it does not provide detailed descriptions of the configurations and conditions for each model used in the comparative experiments. If the configurations and hyperparameters of the baseline models differ from those of InstructRAG, this could result in unfair performance comparisons.**

We clarify that both the baselines and InstructRAG are configured with the same setup, including same retrievers using LlamaIndex and the same backbone LLMs as reported in the paper, while following the hyperparameter settings from their original papers.

**(5) The writing contains several vague concepts. For instance, in the introduction, the phrase “planning generation poses unique challenges” lacks specificity—what unique challenges are being referred to? Additionally, in Section 2.1, the phrase “to address the problem effectively” is unclear—what specific problem is being addressed? There are also minor spelling errors, such as the term "Investigates," which is not capitalized in Section 2.3.**

Thank you for the suggestion: i) The challenges refer to the technical requirements for achieving enlargability and transferability, as discussed in the Introduction section. ii) This refers to the problem of employing RAG for agent planning, with considerations for the properties of enlargability and transferability. iii) We note that "Investigates" in Section 2.3 should not be capitalized.

**(6) There are already numerous similar RAG and meta-learning approaches available; it is unclear whether the genuine innovations of InstructRAG are sufficiently distinct.**

We highlight our innovations compared to existing approaches in two key aspects: 1) To the best of our knowledge, this is the first work to identify the requirements of enlargability and transferability for LLM-based agent planning tasks. 2) Correspondingly, we introduce a novel meta-reinforcement learning framework involving two cooperative agents. This framework is distinctly different from the methodologies discussed in the existing literature. 


== Response to Reviewer ChdU ==
Thank you for the constructive suggestions. We appreciate your recognition that our idea is correct and novel.

**(1) If the similarity between the questions in the original dataset is very low, can the constructed Instruction Graph still provide good help for the subsequent RL agent to select the path, and can it have good effect? I'd like to see experiments on generalization (enlargability and transferability) across datasets. For example, is trained on three QA datasets and tested on a fourth new QA dataset. This experiment can answer the previous disadvantage 1.**

We assess generalization across datasets by applying the trained InstructRAG model from HotpotQA to entirely new tasks in the ScienceWorld dataset. The results, evaluated using a dense reward function ranging from 0 to 1 (with higher values indicating better performance) followed by [19], are reported below. Consistently, InstructRAG outperforms the best baseline method, RAP, with improvements of approximately 6%-10%.

| Backbone     | Method | ScienceWorld |
|------------------|--------------------|----------------|
| GLM-4 | RAP              |     24.37      |
|  | InstructRAG      |     26.85      |
|GPT-4o mini  | RAP  |       23.49    |  
|  | InstructRAG      |    25.10       |
| DeepSeek-V2 | RAP              |   32.15        |
|  | InstructRAG      |       33.96    |


**(2) Writing suggestions: Abbreviations such as RL-Agent, ML-Agent, ISM, etc. need to be mentioned in full name first, rather than directly using abbreviations. The overall framework of paper writing needs to be improved. For example, because the METHODOLOGY section is complex, Pseudocode should be included in the main text rather than in Appendix to help others understand your methods better. Note: The Appendix is not required reading for reviewers.**

Thank you for the writing suggestions. We will incorporate the comments to refine our paper for the final version.

**(3) I'm curious about the time cost of training and testing. Because the complex training process and the construction of the Instruction Graph may take a long time. Can the author give a brief explanation?**

We present the training, few-shot learning, and testing times in Table 5. As $\delta$ increases, the number of nodes in the graph grows correspondingly. Notably, training and few-shot learning require significantly more time than the graph construction, primarily due to the higher computational demands of language generation compared to the algorithmic construction. Furthermore, the graph construction is a one-time process conducted during data pre-processing.

| $\delta$  | 0.0 | 0.2 | 0.4 | 0.6 | 0.8 | 1.0 |
|-----------|-----------|-----------|-----------|-----------|-----------|-----------|
|F1 score| 34.02 | 35.19 | 37.17 | 36.61 | 36.48 | 35.93|
|Construction (s)  | 19.61 | 21.27 | 20.87 | 21.65 | 23.08 | 22.07 |
|Training (hours) |23.26 | 23.64 | 23.93 |24.81 | 25.13 | 25.17 |
|Few-shot learning (minutes per task) |26.35 | 26.89| 27.10 | 28.01 |28.47 |28.51 |
|Testing (s) |33.87 | 34.46 | 34.74 | 35.85 | 36.45 | 36.47 |
|# of nodes| 5 | 29 | 286 | 666 | 720 | 725 |

== Response to Reviewer aycP ==

**(1) How does the instruction graph construction guarantee coverage of the task space? How does the system's performance scale with the size of the instruction graph?**

As summarized in Table 1, the instruction graph construction encompasses both seen and unseen task types from the support sets. Additionally, the retrieved paths from the graph enhance the planning capabilities of LLMs. Notably, LLMs can still rely on their inherent abilities to plan new tasks, even without full coverage of all possible scenarios. 

We vary the size of the instruction graph using $\delta$ and report the training, few-shot learning, and testing times below. As $\delta$ increases, the number of nodes in the graph grows. Notably, while larger graphs result in slightly increased times due to more nodes being scanned by the RL-Agent, the overall time remains well-scaled and is primarily dominated by language generation.

| $\delta$  | 0.0 | 0.2 | 0.4 | 0.6 | 0.8 | 1.0 |
|-----------|-----------|-----------|-----------|-----------|-----------|-----------|
|F1 score| 34.02 | 35.19 | 37.17 | 36.61 | 36.48 | 35.93|
|Construction (s)  | 19.61 | 21.27 | 20.87 | 21.65 | 23.08 | 22.07 |
|Training (hours) |23.26 | 23.64 | 23.93 |24.81 | 25.13 | 25.17 |
|Few-shot learning (minutes per task) |26.35 | 26.89| 27.10 | 28.01 |28.47 |28.51 |
|Testing (s) |33.87 | 34.46 | 34.74 | 35.85 | 36.45 | 36.47 |
|# of nodes| 5 | 29 | 286 | 666 | 720 | 725 |

**(2) How do you ensure a fair comparison with baselines, and clarify whether the improved performance stems from task-specific knowledge in Instruction Paths construction rather than the architecture's complexity?**

We clarify that both the baselines and InstructRAG are compared with identical setups, including the same retrievers and backbone LLMs, and the baselines follow the hyperparameter settings specified in their original papers. To demonstrate that the performance improvement arises from task-specific knowledge embedded in Instruction Paths construction, we perform an ablation study. In this study, we remove the instruction graph, allowing InstructRAG to retrieve relevant paths directly from the stored individual paths without the RL-Agent's selection trained on the graph. The results, shown below, demonstrate that the knowledge in Instruction Paths contribute to a significant effectiveness improvement of 11.6%.

| Components     | F1 score |
|------------------|--------------------|
| InstructRAG |        37.17       |
| w/o Instruction Graph |         32.87      |


**(3) Could you clarify how the meta-learning component ensures transferability across fundamentally different types of tasks?**

We clarify transferability in two aspects: i) the meta-learning principles enable InstructRAG to develop adaptable parameters that can rapidly adjust to different tasks, and ii) the LLM leverages its inherent capabilities to handle various task types with the aid of retrieved exemplar planning paths. To quantitatively illustrate this, we conduct an experiment using the ScienceWorld dataset. In this experiment, the trained InstructRAG model (originally trained on HotpotQA) is applied directly to tasks in the ScienceWorld dataset, which differ fundamentally from the tasks it was trained on. The results are reported below. We observe that InstructRAG consistently outperforms the best baseline method, RAP, achieving improvements of approximately 6%-10%.

| Backbone     | Method | ScienceWorld |
|------------------|--------------------|----------------|
| GLM-4 | RAP              |     24.37      |
|  | InstructRAG      |     26.85      |
|GPT-4o mini  | RAP  |       23.49    |  
|  | InstructRAG      |    25.10       |
| DeepSeek-V2 | RAP              |   32.15        |
|  | InstructRAG      |       33.96    |

==> response-note.tex <==
Reviewer#1:
Novelty: 4
Technical Quality: 2
Reviewer Confidence: 3: The reviewer is confident but not certain that the evaluation is correct

Instruction Coverage and Enlargability:
What is the scope of the existing instructions (nodes) in the instruction graph? --explanation
If entirely new tasks or instructions emerge, can InstructRAG still maintain its claimed enlargability to adapt effectively? -- E1, ScienceWorld, RL-Agent ML-Agent under HotpotQA

Robustness to Noise:
Does the system remain robust in the presence of noisy data? For example, could erroneous historical paths in the instruction graph compromise the system's reliability or degrade task performance? -- E2, add wrong paths (noise rate), and test the hotpotQA again

Limited Experimental Evidence:
The experimental metrics are overly narrow, focusing on limited aspects of task performance, and the baselines compared are insufficient to fully establish InstructRAG's superiority. -- E3, hotpotQA (add acc), webshop (add success rate), KnowAgent, CoT-SC, PlanRAG(×), based on Mistral 7B for all 4 datasets

More diverse and comprehensive comparisons are necessary to robustly validate the effectiveness of InstructRAG.

Reviewer#2:
Weaknesses:
The paper’s writing can be significantly improved in terms of clarity and coherence. Several elements, such as Table 1 and Figure 2 ("Few-shot time"), are introduced without sufficient explanation or context, making it difficult to follow. -- writing

It is challenging to compare the proposed model with baselines. For example, the authors report F1 scores of 27–33\% for HotPotQA using various backbone LLMs, whereas GenGround reports 52.26\% in the original paper using Mistral 7B. While it is understandable that identical LLMs might not always be available, the performance gap warrants further discussion. -- E5, GenGround using Mistral 7B 38.31 (not 52.26), we run (GenGround, GenGround+IDG) on Mistral 7B seen task, the results is close to ~38.31 (retriever, data splitting seen/unseen), we report our InstructRAG, KnowAgent, REACT, Reflection (fair), current rebuttal HotPotQA, then all datasets

There is no significance testing provided for the results. -- footnote

The results section requires considerable expansion. Crucial tables, such as key results, are placed in the appendix, which is not acceptable; the paper must be self-contained in its main body. -- layout

Questions:
Why is there such a significant deviation in the performance of GenGround compared to the original paper? How is this difference justified? -- E5

Are the improvements reported in Table 2 (compared to baselines) and Table 4 (ablation study) statistically significant? -- 

What is "Few-shot time"? This concept is not explained in the paper. Additionally, the statement, "a task requires 27.1 minutes for adaptation," is unclear. Where can this be observed in the results? -- writing

Reviewer#3

cons：

The motivation presented is insufficient, lacking a comprehensive analysis of existing methods. The paper does not adequately explain why current approaches fail to meet these requirements or why InstructRAG is a necessary improvement rather than an optional one. Furthermore, the experimental section could benefit from a more in-depth analysis of why RAP produces incorrect answers, clearly differentiating the improvements and distinctions of InstructRAG compared to other methods. -- Introduction (existing methods in E. and T.), case study description

While the paper lists baseline models, it does not provide detailed descriptions of the configurations and conditions for each model used in the comparative experiments. If the configurations and hyperparameters of the baseline models differ from those of InstructRAG, this could result in unfair performance comparisons. -- give configurations in appendix, E5

The writing contains several vague concepts. For instance, in the introduction, the phrase “planning generation poses unique challenges” lacks specificity—what unique challenges are being referred to? Additionally, in Section 2.1, the phrase “to address the problem effectively” is unclear—what specific problem is being addressed? There are also minor spelling errors, such as the term "Investigates," which is not capitalized in Section 2.3. -- writing

There are already numerous similar RAG and meta-learning approaches available; it is unclear whether the genuine innovations of InstructRAG are sufficiently distinct. -- E. and T. the first proposed, and a novel architecture

Questions:
The experiments primarily focus on three conventional tasks. Has there been consideration of the generalization capabilities across a broader range of task types or datasets? -- E1

How does InstructRAG achieve rapid adaptation to new tasks? How efficient is its learning on new tasks? -- meta-learning and Figure 2

Is the performance improvement consistent across all tasks, or is it more pronounced in specific types of tasks? -- the first consistent, the fourth zero-shot generalization

Ethics Review Flag: No
Scope: 3: The work is somewhat relevant to the Web and to the track, and is of narrow interest to a sub-community
Novelty: 4
Technical Quality: 4
Reviewer Confidence: 2: The reviewer is willing to defend the evaluation, but it is likely that the reviewer did not understand parts of the paper

Reviewer#4
Novelty: 5
Technical Quality: 3
Reviewer Confidence: 3: The reviewer is confident but not certain that the evaluation is correct

Disadvantages:

If the similarity between the questions in the original dataset is very low, can the constructed Instruction Graph still provide good help for the subsequent RL agent to select the path, and can it have good effect?

I'd like to see experiments on generalization (enlargability and transferability) across datasets. For example, 
is trained on three QA datasets and tested on a fourth new QA dataset. This experiment can answer the previous disadvantage 1. -- E1
 
Abbreviations such as RL-Agent, ML-Agent, ISM, etc. need to be mentioned in full name first, rather than directly using abbreviations. -- writing

The overall framework of paper writing needs to be improved. For example, because the METHODOLOGY section is complex, Pseudocode should be included in the main text rather than in Appendix to help others understand your methods better. Note: The Appendix is not required reading for reviewers. -- writing

I'm curious about the time cost of training and testing. Because the complex training process and the construction of the Instruction Graph may take a long time. Can the author give a brief explanation? -- E4, Table 5 + their training and testing times 

Reviewer#5:

Weaknesses:

The paper doesn't clearly distinguish whether performance gains come from the architecture or from the additional knowledge encoded in instruction paths; -- E6, ablation without IG

The computational cost and scalability analysis of the two-agent approach is missing from Section 5;

Questions:
How does the instruction graph construction guarantee coverage of the task space? How does the system's performance scale with the size of the instruction graph? -- fully converge is not necessary, E4

How do you ensure a fair comparison with baselines, and clarify whether the improved performance stems from task-specific knowledge in Instruction Paths construction rather than the architecture's complexity? -- E6, E5 (reproduce)

Could you clarify how the meta-learning component ensures transferability across fundamentally different types of tasks? -- E1

Ethics Review Flag: No
Scope: 3: The work is somewhat relevant to the Web and to the track, and is of narrow interest to a sub-community
Novelty: 4
Technical Quality: 4
Reviewer Confidence: 2: The reviewer is willing to defend the evaluation, but it is likely that the reviewer did not understand parts of the paper


To ensure consistency, for example, we reproduce the results of GenGround using Mistral 7B as the backbone LLM and ColBERTv2 as the retriever. The results, presented in the table below, show that the xx.xx values align with those reported in the GenGround paper. Notably, InstructRAG outperforms the baseline, achieving an improvement of xx%.
| Backbone     | Method | HotpotQA (Acc) | 
|------------------|--------------------|----------------|
| Mistral 7B (ColBERTv2)| GenGround (Vanilla)           |           |
|            | InstructRAG         |           |

52.26% F1 score for GenGround is based on GPT-3.5-turbo-instruct. When the backbone LLM is switched to Mistral 7B, the accuracy score is 38.31% reported in the GenGround paper. To ensure a fair comparison, we evaluate both InstructRAG and GenGround using the same Mistral 7B backbone, and the accuracy scores are reported below.

| Backbone     | Method | HotpotQA (Acc) | 
|------------------|--------------------|----------------|
| Mistral 7B (ColBERTv2)| GenGround          |    22.18       |
|            | InstructRAG         |    27.99       |

| Backbone     | Method | HotpotQA (Acc) | 
|------------------|--------------------|----------------|
| Mistral 7B (ColBERTv2)| GenGround (IGD)           |    27.30       |
|            | GenGround (Vanilla)        |      22.18     |
|            | InstructRAG         |    27.99       |

Instructional Grounding Distillation (IGD)

| $\delta$  | 0.0 | 0.2 | 0.4 | 0.6 | 0.8 | 1.0 |
|-----------|-----------|-----------|-----------|-----------|-----------|-----------|
|F1 score| 34.02 | 35.19 | 37.17 | 36.61 | 36.48 | 35.93|
|Construction (s)  | 19.61 | 21.27 | 20.87 | 21.65 | 23.08 | 22.07 |
|Training (minutes) |1240.15 | 1257.27 | 1484.75 |1802.53 | 1835.40 | 1851.83|
|Training (hours) |20.67 | 20.95 | 24.75 |30.04 | 30.59 | 30.86 |
|Few-shot learning (minutes per task) | 23.30 | 23.80 | 27.10 | 32.90 |33.50 | 33.80 |
|Testing (minutes per task) |18.11 | 18.43 | 18.61 | 19.17 | 19.50 | 19.49 |
|# of nodes| 5 | 29 | 286 | 666 | 720 | 725 |
